New Wine in an Old Bottle -- NeuralPOM: A Hybrid Ocean Forecast Model with Differentiable Dynamics and Staged Learning

Coarse-grid ocean circulation models rely on empirical subgrid parameterizations that struggle to capture mesoscale eddies, whereas purely data-driven neural forecasters accumulate trajectory drift, violate tracer conservation, and damp small-scale variability over extended integrations. Here we present NeuralPOM, a hybrid ocean forecast model that couples differentiable explicit mode-split and semi-implicit free-surface implementations of the Princeton Ocean Model (POM) to a conservation-constrained neural corrector. The three-dimensional primitive-equation solver advances the ocean state, while the neural network periodically updates the physical fields at high-frequency (1 h) or low-frequency (1 day) intervals under volume, heat, and salt conservation constraints. Using a fine-grid reference dataset exceeding 100,000 model days in a wind-driven double-gyre basin, we introduce a three-stage training procedure comprising offline single-step pretraining, multi-step differentiable training through the ocean solver, and multi-day closed-loop rollout training. Over 100-day forecasts, NeuralPOM reduces errors across all prognostic fields relative to coarse-grid physical closures and direct neural forecasters, preserving mesoscale kinetic energy while improving eddy phase alignment. Controlled ablations show that closed-loop training suppresses multi-day drift, whereas backpropagating gradients through the differentiable solver stabilizes high-frequency coupling. Finally, because high-frequency tracer updates can introduce density anomalies via the equation of state that excite spurious baroclinic pressure gradients, we introduce Density-Normal Damping (DND) to attenuate the density-modifying (diapycnal) tracer component while retaining the density-compensated (isopycnal) correction.

==> data/ai_baselines/table_1_100_rows.tex <==
\texttt{Smagorinsky} & \underline{0.07926} & 0.08197 & \underline{0.11970} & \underline{0.29351} & \underline{0.03382} \\
\midrule
Triton Pre & 0.09935 & 0.09526 & 0.21544 & 0.79294 & 0.21825 \\
Triton Post & 0.08886 & 0.08663 & 0.14570 & 0.36668 & 0.10914 \\
\midrule
ResUNet Pre & 0.10189 & 0.09767 & 0.16460 & 0.45770 & 0.12531 \\
ResUNet Post & 0.08267 & 0.08401 & 0.12812 & 0.60935 & 0.22609 \\
\midrule
SimVP Pre & 0.09434 & 0.09123 & 0.22382 & 0.79226 & 0.21567 \\
SimVP Post & 0.08452 & \underline{0.08180} & 0.13804 & 0.63266 & 0.25703 \\
\midrule
ConvLSTM Pre & 0.10088 & 0.10351 & 0.29508 & 0.96630 & 0.22385 \\
ConvLSTM Post & 0.10222 & 0.09665 & 0.18062 & 0.51404 & 0.10723 \\
\midrule
PastNet Pre & 0.14249 & 0.12674 & 0.23017 & 0.61166 & 0.17605 \\
PastNet Post & 0.10278 & 0.10150 & 0.17001 & 0.77017 & 0.26912 \\
\midrule
NeuralPOM Post-\texttt{DND} (ours) & \cellcolor{physics!14}\textbf{0.07415} & \cellcolor{physics!14}\textbf{0.07789} & \cellcolor{physics!14}\textbf{0.11227} & \cellcolor{physics!14}\textbf{0.26537} & \cellcolor{physics!14}\textbf{0.02822} \\


==> data/ai_baselines/table_1_50_rows.tex <==
\texttt{Smagorinsky} & \underline{0.05715} & 0.06125 & \underline{0.08291} & \underline{0.20676} & \underline{0.02327} \\
\midrule
Triton Pre & 0.08046 & 0.08143 & 0.16975 & 0.60555 & 0.16690 \\
Triton Post & 0.06722 & 0.06694 & 0.11266 & 0.29419 & 0.09654 \\
\midrule
ResUNet Pre & 0.08042 & 0.07820 & 0.12440 & 0.35888 & 0.09838 \\
ResUNet Post & 0.05796 & \underline{0.05934} & 0.08642 & 0.43161 & 0.17765 \\
\midrule
SimVP Pre & 0.08407 & 0.08155 & 0.19107 & 0.68022 & 0.18472 \\
SimVP Post & 0.06137 & 0.06152 & 0.10150 & 0.51095 & 0.22896 \\
\midrule
ConvLSTM Pre & 0.10115 & 0.10333 & 0.30347 & 0.94709 & 0.21542 \\
ConvLSTM Post & 0.07765 & 0.07741 & 0.13209 & 0.39224 & 0.08424 \\
\midrule
PastNet Pre & 0.11779 & 0.11206 & 0.18938 & 0.54899 & 0.18091 \\
PastNet Post & 0.08345 & 0.08456 & 0.13818 & 0.72325 & 0.26158 \\
\midrule
NeuralPOM Post-\texttt{DND} (ours) & \cellcolor{physics!14}\textbf{0.04813} & \cellcolor{physics!14}\textbf{0.05282} & \cellcolor{physics!14}\textbf{0.06935} & \cellcolor{physics!14}\textbf{0.16586} & \cellcolor{physics!14}\textbf{0.01769} \\


==> data/ai_baselines/table_51_100_rows.tex <==
\texttt{Smagorinsky} & \underline{0.09644} & 0.09841 & \underline{0.14759} & \underline{0.35992} & \underline{0.04179} \\
\midrule
Triton Pre & 0.11518 & 0.10732 & 0.25301 & 0.94383 & 0.25964 \\
Triton Post & 0.10619 & 0.10261 & 0.17253 & 0.42704 & 0.12042 \\
\midrule
ResUNet Pre & 0.11957 & 0.11386 & 0.19674 & 0.53868 & 0.14740 \\
ResUNet Post & 0.10154 & 0.10292 & 0.15925 & 0.74587 & 0.26585 \\
\midrule
SimVP Pre & 0.10359 & 0.09997 & 0.25235 & 0.89031 & 0.24270 \\
SimVP Post & 0.10257 & \underline{0.09798} & 0.16676 & 0.73448 & 0.28231 \\
\midrule
ConvLSTM Pre & 0.10062 & 0.10370 & 0.28644 & 0.98514 & 0.23197 \\
ConvLSTM Post & 0.12194 & 0.11266 & 0.21862 & 0.61207 & 0.12609 \\
\midrule
PastNet Pre & 0.16349 & 0.13989 & 0.26474 & 0.66849 & 0.17105 \\
PastNet Post & 0.11901 & 0.11599 & 0.19676 & 0.81440 & 0.27646 \\
\midrule
NeuralPOM Post-\texttt{DND} (ours) & \cellcolor{physics!14}\textbf{0.09317} & \cellcolor{physics!14}\textbf{0.09666} & \cellcolor{physics!14}\textbf{0.14283} & \cellcolor{physics!14}\textbf{0.33666} & \cellcolor{physics!14}\textbf{0.03577} \\

